Joint Communication and Sensing with Bipartite Entanglement over Bosonic Channels

We consider a joint communication and sensing problem over an optical link in which a low-power transmitter simultaneously communicates with a receiver and identifies the range of a defect producing a backscattered signal. We model the system as a lossy thermal-noise bosonic channel, in which the target location, modeled as a beamsplitter, affects the timing of the backscattered signal. Motivated by the envisioned deployment of entanglement-enabled quantum networks, we allow the transmitter to exploit shared entanglement to assist both sensing and communication. Since entanglement is known to enhance sensing, as demonstrated in Quantum Illumination (QI), and to increase communication rates through entanglement-assisted communication, the transmitter faces a trade-off in allocating its entanglement resources between the two tasks. Our main result is a characterization of these trade-offs in the form of an achievable rate/error-exponent region, which can outperform time-sharing and demonstrates a quantum advantage.

==> Acronyms.tex <==
\acrodef{ACDIS}[ACDIS]{Adaptive Communication Decision and Information Systems}
\acrodef{AEP}{Asymptotic Equipartition Property}
\acrodef{AoA}{Angle of Arrival}
\acrodef{AWGN}{Additive White Gaussian Noise}
\acrodef{AVC}[AVC]{Arbitrarily Varying Channel}
\acrodef{BER}{Bit-Error-Rate}
\acrodef{BEC}{Binary Erasure Channel}
\acrodef{BPSK}{Binary Phase-Shift Keying}
\acrodef{BSC}{Binary Symmetric Channel}
\acrodef{BICM}[BICM]{Bit-Interleaved Coded-Modulation}
\acrodef{C3MSV}[C3MSV]{Coupled Three-Mode Squeezed Vacuum}
\acrodef{CDF}[CDF]{Cumulative Distribution Function}
\acrodef{CGF}[CGF]{Cumulant Generating Function}
\acrodef{CLT}[CLT]{Central Limit Theorem}
\acrodef{CSI}[CSI]{Channel State Information}
\acrodef{DMC}[DMC]{Discrete Memoryless Channel}
\acrodef{DMS}[DMS]{Discrete Memoryless Source}
\acrodef{ERM}[ERM]{Empirical Risk Minimization}
\acrodef{FER}[FER]{Frame Error Rate}
\acrodef{ICA}[ICA]{Independent Component Analysis}
\acrodef{iid}[i.i.d.]{independent and identically distributed}
\acrodef{IoT}[IoT]{Internet of Things}
\acrodef{KKT}[KKT]{Karush-Kuhn Tucker}
\acrodef{LASSO}[LASSO]{Least Absolute Shrinkage and Selection Operator}
\acrodef{LPD}[LPD]{Low Probability of Detection}
\acrodef{LDPC}[LDPC]{Low-Density Parity-Check}
\acrodef{LLMS}[LLMS]{Linear Least Mean Square}
\acrodef{LMS}[LMS]{Least Mean Square}
\acrodef{MAC}[MAC]{multiple-access channel}
\acrodef{MGF}[MGF]{Moment Generating Function}
\acrodef{MLC}[MLC]{Multi-Level Coding}
\acrodef{MLE}[MLE]{Maximum Likelihood Estimate}
\acrodef{MIMO}[MIMO]{Multiple-Input Multiple-Output}
\acrodef{MISO}{Multiple-Input Single-Output}
\acrodef{MSD}[MSD]{Multi-Stage Decoding}
\acrodef{MMSE}[MMSE]{Minimum Mean-Square Error}
\acrodef{NPS}[NPS]{No Passive Signature}
\acrodef{PAC}[PAC]{Probably Approximately Correct}
\acrodef{PCA}[PCA]{Principal Component Analysis}
\acrodef{PDF}[PDF]{Probability Density Function}
\acrodef{PMF}[PMF]{Probability Mass Function}
\acrodef{POVM}[POVM]{Positive Operator-Valued Measure}
\acrodef{PVM}[PVM]{Projection-Valued Measure}
\acrodef{PPM}[PPM]{Pulse Position Modulation}
\acrodef{PSD}{Power Spectral Density}
\acrodef{PSK}{Phase Shift Keying}
\acrodef{QI}{Quantum Illumination}
\acrodef{QKD}{Quantum Key Distribution}
\acrodef{ROC}{Receiver Operating Characteristic}
\acrodef{c-q}{Classical-Quantum}
\acrodef{CVQKD}{Continuous-Variable \ac{QKD}}
\acrodef{QKF}[QMF]{Quantum-Memory Free}
\acrodef{QPSK}{Quadrature Phase-Shift Keying}
\acrodef{QSDC}[QSDC]{Quantum Secure Direct Communication}
\acrodef{RV}{random variable}
\acrodef{SIMO}{Single-Input Multiple-Output}
\acrodef{SNR}{Signal-to-Noise Ratio}
\acrodef{SVM}[SVM]{Support Vector Machine}
\acrodef{TMSV}[TMSV]{Two-Mode Squeezed Vaccum}
\acrodef{TPCP}{Trace-Preserving Completely-Positive}
\acrodef{wrt}[w.r.t.]{with respect to}
\acrodef{WSS}{Wide Sense Stationary}


==> arcom_functions.tex <==
%---------------------------------------------
% Probability, statistics, information theory
%---------------------------------------------

\renewcommand{\P}[2][]{{\mathbb{P}_{#1}}{\left(#2\right)}} % probability measure
\newcommand{\p}[2][]{\ensuremath{p_{#1}\!\left({#2}\right)}} % probability mass or density
\newcommand{\E}[2][]{{\mathbb{E}_{#1}}{\left(#2\right)}} % Expectation of a random variable      
\newcommand{\Var}[1]{{\text{\textnormal{Var}}{\left(#1\right)}}} % variance      
\newcommand{\avgD}[3][]{{\mathbb{D}_{#1}}\!\left(\smash{#2}\,\middle\Vert\,\smash{#3}\right)} % divergence
\newcommand{\avgDs}[4][]{{\mathbb{D}^{#1}_{#2}}\!\left(\smash{#3}\,\middle\Vert\,\smash{#4}\right)} % smooth-type relative entropy
\newcommand{\avgDMs}[3][]{{\mathbb{D}^{#1}_{\text{\textnormal{max}}}}\!\left(\smash{#2}\,\middle\Vert\,\smash{#3}\right)} % smooth max relative entropy
\newcommand{\avgDHs}[3][]{{\mathbb{D}^{#1}_{\text{\textnormal{H}}}}\!\left(\smash{#2}\,\middle\Vert\,\smash{#3}\right)} % smooth hypothesis testing relative entropy
\newcommand{\D}[3][]{{\mathbb{D}_{#1}}\!\left(#2\,\middle\Vert\,#3\right)} % divergence
%\newcommand{\D}[2]{{{\mathbb{D}}\!\left({#1\Vert#2}\right)}} % old divergence - obsolete
\newcommand{\V}[1]{{{\mathbb{V}}\!\left(\smash{#1}\right)}} % total variation
\newcommand{\Ks}[2]{{\bbchi}^2\!\left(#1\,\middle\Vert\,#2\right)} % chi-square distance
\newcommand{\supp}[1]{{{\textnormal{supp}\left(#1\right)}}} % support of random variable
\newcommand{\avgI}[1]{{{\mathbb{I}}\!\left(#1\right)}} % mutual information
\newcommand{\avgIM}[2]{{{\tilde{\mathbb{I}}^{#1}_{\text{\textnormal{max}}}}\!\left(#2\right)}} % max mutual information
\newcommand{\avgIH}[2]{{{\tilde{\mathbb{I}}^{#1}_{\text{\textnormal{H}}}}\!\left(#2\right)}} % hypothesis testing mutual information
\newcommand{\I}[2]{{{\mathbb{I}}\!\left(#1;#2\right)}} % mutual information (two params)
\newcommand{\avgH}[1]{{\mathbb{H}}\!\left(#1\right)}
\renewcommand{\H}[1]{{\mathbb{H}}\!\left(#1\right)}
\newcommand{\Hb}[1]{{h_b}\left(#1\right)} % Binary entropy function
\newcommand{\splx}[1]{\Delta\left(#1\right)} % probability simplex
%\newcommand{\avgIk}[2]{\mathbb{I}_{#1}\left(#2\right)} % old mutual information - obsolete
%\newcommand{\I}[1]{{\randomvalue{I}}{\left(#1\right)}} % old mutual information - obsolete
%\renewcommand{\H}[1]{{\randomvalue{H}}\!\left(#1\right)} % old entropy - obsolete
\newcommand{\h}[1]{{{h}}\left(#1\right)} % differential entropy
\newcommand{\plimsup}[2][n\rightarrow\infty]{\underset{#1}{\mbox{\textnormal{p-limsup}}\;}{#2}} % plim sup
% \newcommand{\plimsup}[2][n\rightarrow\infty]{\underset{#1}{\overline{\textnormal{p-lim}}\;}{#2}}
% plim inf
\newcommand{\pliminf}[2][n\rightarrow\infty]{\underset{#1}{\mbox{\textnormal{p-liminf}}\;}{#2}}
% \newcommand{\pliminf}[2][n\rightarrow\infty]{\underset{#1}{\underline{\textnormal{p-lim}}\;}{#2}}
\newcommand{\plim}[2][n\rightarrow\infty]{\underset{#1}{\mbox{p-lim}\;}{#2}} % plim (convergence in probability)
\newcommand{\proddist}{%
  \mathchoice{\raisebox{1pt}{$\displaystyle\otimes$}}
             {\raisebox{1pt}{$\otimes$}}
             {\raisebox{0.5pt}{\scalebox{0.7}{$\scriptstyle\otimes$}}}
             {\raisebox{0.4pt}{\scalebox{0.6}{$\scriptscriptstyle\otimes$}}}}
\newcommand{\pn}{{\proddist n}} % product distribution

%---------------------------------------------
% Coding theory
% ---------------------------------------------

\newcommand{\GF}[1]{\ensuremath{\mbox{GF}(#1)}} % Galois field
\newcommand{\F}[1]{\ensuremath{\mathbb{F}_{#1}}} % Field
\newcommand{\dH}[1]{\ensuremath{\mbox{d}_{\mbox{\tiny H}}(#1)}} % Hamming distance
\newcommand{\wt}[1]{\ensuremath{\mbox{wt}(#1)}} % Weight of a vector

%---------------------------------------------
% General commands
% ---------------------------------------------

\newcommand{\card}[1]{\ensuremath{\left|{#1}\right|}} % Cardinality of a set
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}} % Absolute value        
\newcommand{\norm}[2][]{\ensuremath{{\left\Vert{#2}\right\Vert}_{#1}}} % Norm
\newcommand{\eqdef}{\ensuremath{\triangleq}} % Defined by equality
\newcommand{\intseq}[2]{\ensuremath{\llbracket{#1},{#2}\rrbracket}} % Sequence of integers
\newcommand{\set}[1]{\ensuremath{\left\{{#1}\right\}}} % set
\newcommand{\indic}[1]{\ensuremath{\mathds{1}\!\left\{#1\right\}}} % indicator function
\newcommand{\dd}{\text{\textnormal{d}}} % differential operator as in dx
\renewcommand{\leq}{\leqslant} % redefines <=
\renewcommand{\geq}{\geqslant} % redefines >=
\newcommand{\argmin}{\mathop{\text{argmin}}} % argmin
\newcommand{\argmax}{\mathop{\text{argmax}}} % argmax
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\bra}[1]{\left\langle #1 \right|}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}

%---------------------------------------------
% Matrix operations
% ---------------------------------------------

\newcommand{\mat}[2]{\left[\begin{array}{#1}#2\end{array}\right]} % shortcut to construct array
\newcommand{\tr}[2][]{\ensuremath{\text{\textnormal{tr}}_{#1}\left(#2\right)}}  % Trace
\newcommand{\rk}[1]{\ensuremath{\text{\textnormal{rank}}\left(#1\right)}}  % Rank
\renewcommand{\det}[1]{{\left|{#1}\right|}}                              % Det
\renewcommand{\ker}[1]{\ensuremath{\text{\textnormal{Ker}}\left(#1\right)}}  % Kernel
\newcommand{\range}[1]{\ensuremath{\text{\textnormal{range}}}\left(#1\right)} % range
\newcommand{\crange}[1]{\overline{\ensuremath{\text{\textnormal{range}}}}\left(#1\right)} % closure of range


%---------------------------------------------
% Others
% ---------------------------------------------

\newcommand{\mycomment}[1]{\marginpar{\raggedright\footnotesize\PencilRightDown~\textcolor{red}{#1}}}
\newcommand{\mypar}[2]{\noindent\textbf{$\blacktriangleright$~#1}~{#2}}
\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}\xspace} % citation needed command (to clearly show something missing)

%---------------------------------------------
% Legacy commands - somewhat obsolete
% ---------------------------------------------

\newcommand{\cl}[1]{\ensuremath{\text{\textnormal{cl}}\!\left(#1\right)}}% closure
\newcommand{\info}[2]{\ensuremath{\mathbb{I}\!\left({#1};{#2}\right)}}
\newcommand{\rvinfo}[2]{\ensuremath{\mathssf{i}\!\left({#1};{#2}\right)}}
\newcommand{\KLdiv}[2]{\ensuremath{\mathbb{D}\!\left({#1}||{#2}\right)}}
\newcommand{\entropy}[1]{\ensuremath{\mathbb{H}\!\left({#1}\right)}}
\newcommand{\diffentropy}[1]{\ensuremath{h\!\left({#1}\right)}}
\newcommand{\expect}[2][]{\ensuremath{\mathbb{E}_{#1}{\left\{#2\right\}}}}
\newcommand{\dprob}[2][]{\ensuremath{\mbox{\textnormal{Pr}}_{#1}{\left[{#2}\right]}}}
\newcommand{\cprob}[2][]{\ensuremath{p_{#1}\left({#2}\right)}}
\newcommand{\sts}[3]{T_{#1}^{#2}\!(#3)} % typical set
\newcommand{\wts}[2]{\ensuremath{A_{#1}^{(#2)}}} % typical set
\newcommand{\stsne}[3]{S_{\left[#1\right]}^{#2}\!(#3)} % another typical set
\newcommand{\vct}[1]{\ensuremath{\mathbf{#1}}} % vector
\newcommand{\vctlist}[3]{\ensuremath{\left(#1_{#2},\dots,#1_{#3}\right)}} % vector expanded
%\newcommand{\setlist}[3][\dots]{\ensuremath{\left\{#2,#1,#3\right\}}}

%% mydef
\newcommand{\limn}[2][n\rightarrow\infty]{\underset{#1}{\mbox{\textnormal{lim}}\;}{#2}}
\renewcommand{\liminf}[2][n\rightarrow\infty]{\underset{#1}{\mbox{\textnormal{liminf}}\;}{#2}}
\renewcommand{\limsup}[2][n\rightarrow\infty]{\underset{#1}{\mbox{\textnormal{limsup}}\;}{#2}}
\newcommand{\N}[2]{\calN\left({#1},{#2}\right)}
\newcommand{\blog}[1]{\mbox{\textnormal{log}}\left({#1}\right)}
\newcommand{\Qfunc}[1]{Q\left({#1}\right)}
\newcommand{\invQfunc}[1]{Q^{-1}\left({#1}\right)}
% matrix constructed by vct
% ex: \matvct{x}{1}{n}
\newcommand{\matvct}[3]{\ensuremath{\left[#1_{#2}~\dots~#1_{#3}\right]}}
\newcommand{\diag}[1]{\textnormal{diag}\left(#1\right)}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\chidist}[3]{{\bbchi}_{#1}\!\left(#2\,\middle\Vert\,#3\right)} % chi-square distance
% \newcommand{\wt}[1]{\ensuremath{\text{\textnormal{wt}}\!\left(#1\right)}}
\newcommand{\srH}[3]{\mathbb{H}_{#1}^{#2}\left(#3\right)}

% --------------------------
%  Quantnum
%  --------------------------

\newcommand{\Pdist}[1]{\ensuremath{\text{\textnormal{P}}}\left(#1\right)} % Purified distance
\newcommand{\Fidelity}[1]{\ensuremath{\text{\textnormal{F}}}\left(#1\right)} % Fidelity
\newcommand{\rFidelity}[1]{\ensuremath{\sqrt{\text{\textnormal{F}}}}\left(#1\right)} % Square-root Fidelity
\newcommand{\ball}[2][]{\calB^{#1}\left(#2\right)} % epsilon-ball

==> arcom_notation.tex <==
%% Definitions of random variable fonts.
\DeclareMathAlphabet{\eurm}{U}{eur}{m}{n}
\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\DeclareMathAlphabet{\mathcsf}{OT1}{cmss}{sbc}{n}% condensed sans serif

%% font change
%\newcommand{\samplevalue}[1]{#1}
%\newcommand{\randomvalue}[1]{\eurm{#1}}

%% case change
\newcommand{\samplevalue}[1]{{\lowercase{#1}}}
\newcommand{\randomvalue}[1]{{\uppercase{#1}}}

% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}  
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}


%% Random variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
\newcommand{\rvA}{{\randomvalue{A}}}	% A
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\rvB}{{\randomvalue{B}}}
\newcommand{\rvbB}{{\mathbsf{B}}}
\newcommand{\rvC}{{\randomvalue{C}}}
\newcommand{\rvD}{{\randomvalue{D}}}
\newcommand{\rvE}{{\randomvalue{E}}}
\newcommand{\rvF}{{\randomvalue{F}}}
\newcommand{\rvG}{{\randomvalue{G}}}
\newcommand{\rvH}{{\randomvalue{H}}}
\newcommand{\rvI}{{\randomvalue{I}}}
\newcommand{\rvJ}{{\randomvalue{J}}}
\newcommand{\rvK}{{\randomvalue{K}}}
\newcommand{\rvL}{{\randomvalue{L}}}	% L
\newcommand{\rvM}{{\randomvalue{M}}}	% M
\newcommand{\rvN}{{\randomvalue{N}}}	% N
\newcommand{\rvQ}{{\randomvalue{Q}}}	% R
\newcommand{\rvR}{{\randomvalue{R}}}	% R
\newcommand{\rvS}{{\randomvalue{S}}}	% S
\newcommand{\rvT}{{\randomvalue{T}}}	% S
\newcommand{\rvU}{{\randomvalue{U}}}	% U
\newcommand{\rvV}{{\randomvalue{V}}}	% V
\newcommand{\rvW}{{\randomvalue{W}}}	% W
\newcommand{\rvX}{{\randomvalue{X}}}  	% X
\newcommand{\rvY}{{\randomvalue{Y}}}	% Y
\newcommand{\rvZ}{{\randomvalue{Z}}}	% Z

\newcommand{\rva}{{\randomvalue{a}}}	% a
\newcommand{\sva}{{\samplevalue{a}}}	% a
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\rvb}{{\randomvalue{b}}}	% b
\newcommand{\svb}{{\samplevalue{b}}}	% b
%\newcommand{\rvbh}{\hat{\rvb}}
\newcommand{\rvc}{{\randomvalue{c}}}	% c
\newcommand{\svc}{{\samplevalue{c}}}	% c
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\rvd}{{\randomvalue{d}}}	% d
\newcommand{\rvbd}{{\mathbsf{d}}}
\newcommand{\rve}{{\randomvalue{e}}}	% e
\newcommand{\rvbe}{{\mathbsf{e}}}
\newcommand{\rvf}{{\randomvalue{f}}}	% f
\newcommand{\rvg}{{\randomvalue{g}}}
\newcommand{\rvh}{{\randomvalue{h}}}	% h
\newcommand{\svh}{{\samplevalue{h}}}	% c
\newcommand{\rvbh}{{\mathbsf{h}}}
\newcommand{\rvi}{{\randomvalue{i}}}	% i
\newcommand{\svi}{{\samplevalue{i}}}	% i
\newcommand{\rvk}{{\randomvalue{k}}}	% k
\newcommand{\svk}{{\samplevalue{k}}}	% k
\newcommand{\rvl}{{\randomvalue{l}}}
\newcommand{\svl}{{\samplevalue{l}}}
\newcommand{\rvm}{{\randomvalue{m}}}	% m
\newcommand{\svm}{{\samplevalue{m}}}	% m
\newcommand{\rvmh}{\hat{\rvm}}
\newcommand{\rvbm}{{\mathbsf{m}}}
\newcommand{\rvbmh}{\hat{\rvbm}}
\newcommand{\rvn}{{\randomvalue{n}}}	% n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvq}{{\randomvalue{q}}}	% q
\newcommand{\svq}{{\samplevalue{q}}}
\newcommand{\rvr}{{\randomvalue{r}}}	% r
\newcommand{\svr}{{\samplevalue{r}}}
\newcommand{\rvs}{{\randomvalue{s}}}	% s
\newcommand{\svs}{{\samplevalue{s}}}
\newcommand{\rvsh}{\hat{\rvs}}
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\rvt}{{\randomvalue{t}}}	% t
\newcommand{\svt}{{\samplevalue{t}}}
\newcommand{\rvu}{{\randomvalue{u}}}	% u
\newcommand{\svu}{{\samplevalue{u}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\rvv}{{\randomvalue{v}}}	% v
\newcommand{\svv}{{\samplevalue{v}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvw}{{\randomvalue{w}}}	% w
\newcommand{\svw}{{\samplevalue{w}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvwh}{\hat{\rvw}}
\newcommand{\rvx}{{\randomvalue{x}}}	% x
\newcommand{\svx}{{\samplevalue{x}}}
\newcommand{\rvxh}{\hat{\rvx}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvy}{{\randomvalue{y}}}	% y
\newcommand{\svy}{{\samplevalue{y}}}
\newcommand{\rvyh}{{\hat{\rvy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvz}{{\randomvalue{z}}}	% z
\newcommand{\rvzh}{\hat{\rvz}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svz}{{\samplevalue{z}}}
% Handle uppercase Greek differently
\newcommand{\rvDelta}{\ssfDelta}
\newcommand{\rvbDelta}{\bsfDelta}
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\rvbPh}{\bsfPhi}

% Caligraphy
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\bfzero}{\mathbf{0}}
\newcommand{\bfone}{\mathbf{1}}

\newcommand{\bflambda}{\boldsymbol{\lambda}}
\newcommand{\bfalpha}{\boldsymbol{\alpha}}
\newcommand{\bfbeta}{\boldsymbol{\beta}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}
\newcommand{\bftheta}{\boldsymbol{\theta}}
\newcommand{\bfrho}{\boldsymbol{\rho}}
\newcommand{\bfxi}{\boldsymbol{\xi}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbchi}{\mathbb{\chi}}

%% mydef
%\newcommand{\bbN}{\mathbb{N}}
\newcommand{\Pinn}{P_0}
\newcommand{\Pinf}{P_n}
\newcommand{\Qinn}{Q_0}
\newcommand{\Qinf}{Q_n}
\newcommand{\Qcode}{\widehat{Q}}

\newcommand{\QinfH}{Q_{\vct{H}}}
\newcommand{\QinfHn}{\QinfH^{\otimes n}}
\newcommand{\QinfL}{\widetilde{Q}_{\vct{\Lambda}}}
\newcommand{\QinfLn}{\QinfL^{\otimes n}}

\newcommand{\QinftH}{Q_{\widetilde{\vct{H}}}}
\newcommand{\QinftHn}{\QinftH^{\otimes n}}
\newcommand{\QinfHw}{Q_{\vct{H}_w}}
\newcommand{\QinfHwn}{\QinfHw^{\otimes n}}
\newcommand{\QinftL}{\widetilde{Q}_{\widetilde{\vct{\Lambda}}}}
\newcommand{\QinftLn}{\QinftL^{\otimes n}}

\newcommand{\PiQn}{\Pi_{\vct{Q}_n}}
\newcommand{\PiPn}{\Pi_{\vct{P}_n}}
\newcommand{\PiQnn}{\Pi_{\vct{Q}_n}^{\otimes n}}
\newcommand{\PiPnn}{\Pi_{\vct{P}_n}^{\otimes n}}
\newcommand{\Pinnn}{P_0^{\otimes n}}
\newcommand{\Pinfn}{P_n^{\otimes n}}
\newcommand{\Qinnn}{Q_0^{\otimes n}}
\newcommand{\Qinfn}{Q_n^{\otimes n}}
\newcommand{\Qcoden}{\widehat{Q}^n}

\newcommand{\parPinn}{\widetilde{P}_0}
\newcommand{\parPinf}{\widetilde{P}_n}
\newcommand{\parQinn}{\widetilde{Q}_0}
\newcommand{\parQinf}{\widetilde{Q}_n}

\newcommand{\parPinnn}{\widetilde{P}_0^{\otimes n}}
\newcommand{\parPinfn}{\widetilde{P}_n^{\otimes n}}
\newcommand{\parQinnn}{\widetilde{Q}_0^{\otimes n}}
\newcommand{\parQinfn}{\widetilde{Q}_n^{\otimes n}}

\newcommand{\parjPinn}{\widetilde{P}_{0,j}}
\newcommand{\parjPinf}{\widetilde{P}_{n,j}}
\newcommand{\parjQinn}{\widetilde{Q}_{0,j}}
\newcommand{\parjQinf}{\widetilde{Q}_{n,j}}

\newcommand{\parjPinnn}{\widetilde{P}_{0,j}^{\otimes n}}
\newcommand{\parjPinfn}{\widetilde{P}_{n,j}^{\otimes n}}
\newcommand{\parjQinnn}{\widetilde{Q}_{0,j}^{\otimes n}}
\newcommand{\parjQinfn}{\widetilde{Q}_{n,j}^{\otimes n}}

%% precoding variable
\newcommand{\parVarX}{\tilde{\vct{X}}}
\newcommand{\parVarY}{\tilde{\vct{Y}}}
\newcommand{\parVarZ}{\tilde{\vct{Z}}}
\newcommand{\parVarx}{\tilde{\vct{x}}}
\newcommand{\parVary}{\tilde{\vct{y}}}
\newcommand{\parVarz}{\tilde{\vct{z}}}

\newcommand{\hermittian}{\intercal}

\newcommand{\Ww}{W_{\vct{Z}|\vct{X}}}
\newcommand{\Wwn}{W_{\vct{Z}|\vct{X}}^{\otimes n}}
\newcommand{\tWwn}{\widetilde{W}_{\vct{Z}|\vct{X}}^{\otimes n}}

\newcommand{\Wb}{W_{\vct{Y}|\vct{X}}}
\newcommand{\Wbn}{W_{\vct{Y}|\vct{X}}^{\otimes n}}
\newcommand{\parWw}{W_{\tilde{\vct{Z}}|\tilde{\vct{X}}}}
\newcommand{\parWwn}{W_{\tilde{\vct{Z}}|\tilde{\vct{X}}}^{\otimes n}}
\newcommand{\partWw}{\widetilde{W}_{\tilde{\vct{Z}}|\tilde{\vct{X}}}}
\newcommand{\partWwn}{\widetilde{W}_{\tilde{\vct{Z}}|\tilde{\vct{X}}}^{\otimes n}}
\newcommand{\parWb}{W_{\tilde{\vct{Y}}|\tilde{\vct{X}}}}
\newcommand{\parWbn}{W_{\tilde{\vct{Y}}|\tilde{\vct{X}}}^{\otimes n}}

\newcommand{\Pirhonj}{\Pi_{\rho_{n,j}}}
\newcommand{\Pirhonjn}{\Pirhonj^{\otimes n}}
\newcommand{\parjWw}{W_{\tilde{Z}^{(j)}|\tilde{X}^{(j)}}}
\newcommand{\parjWwn}{W_{\tilde{Z}^{(j)}|\tilde{X}^{(j)}}^{\otimes n}}
\newcommand{\parjtWw}{\widetilde{W}_{\tilde{Z}^{(j)}|\tilde{X}^{(j)}}}
\newcommand{\parjtWwn}{\widetilde{W}_{\tilde{Z}^{(j)}|\tilde{X}^{(j)}}^{\otimes n}}
\newcommand{\parjWb}{W_{\tilde{Y}^{(j)}|\tilde{X}^{(j)}}}
\newcommand{\parjWbn}{W_{\tilde{Y}^{(j)}|\tilde{X}^{(j)}}^{\otimes n}}

\newcommand{\invQdelta}{\invQfunc{\frac{1-\delta_n}{2}}}

